Diverse Unionable Tuple Search: Novelty-Driven Discovery in Data Lakes [Technical Report]

Unionable table search techniques input a query table from a user and search for data lake tables that can contribute additional rows to the query table. The definition of unionability is generally based on similarity measures which may include similarity between columns (e.g., value overlap or semantic similarity of the values in the columns) or tables (e.g., similarity of table embeddings). Due to this and the large redundancy in many data lakes (which can contain many copies and versions of the same table), the most unionable tables may be identical or nearly identical to the query table and may contain little new information. Hence, we introduce the problem of identifying unionable tuples from a data lake that are diverse with respect to the tuples already present in a query table. We perform an extensive experimental analysis of well-known diversity algorithms applied to this novel problem and identify a gap that we address with a novel, clustering-based tuple diversity algorithm called DUST. DUST uses a novel embedding model to represent unionable tuples that outperforms other tuple representation models by at least 15 % when representing unionable tuples. Using real data lake benchmarks, we show that our diversification algorithm is more than six times faster than the most efficient diversification baseline. We also show that it is more effective in diversifying unionable tuples than existing diversification algorithms.

==> sections/model-architecture.tex <==
\section{\ourmethod Implementation}
\label{section:model-architecture}
\begin{figure*}[ht]
  \includegraphics[scale = 0.5]{figures/dust_block_diagram.pdf}
  \caption{Diverse Unionable Tuple Search (\ourmethod)}
\label{fig:dust_block_diagram}
\end{figure*}
Now we detail our proposed solution for the Diverse Unionable Tuple Search Problem. Note that we expect all k tuples in the output set to be unionable with the query table, and they are diverse with respect to each other. For diversity, given a unionability embedding space, we want to ensure that the tuples are evenly distributed throughout the space such that the distance between each pair of tuples is maximized.
We propose to solve this problem in two steps. First, we search for a set of data lake tuples $S$ that are unionable with the tuples in the query table. For this, we build a fine-tuned BERT-based model~\cite{2019_devlin_bert} that embeds each tuple in a unionability space. Then in the second step, we select k tuples from $S$ such that they are diverse with respect to the query tuples. Prior work showed that the problem of finding a subset of k diverse items from a set of relevant items is computationally hard~\cite{2011_vieira_divdb}. So, we will propose a clustering-based approach that efficiently computes an approximate solution.

\subsection{Tuple Search}
\subsection{Column Alignment}
\subsection{Tuple Representation}
\subsection{Tuple Diversification}

==> sections/tuple-search.tex <==
\section{Unionable Tuple Search}
\label{section:unionable_tuple_search}

We now explain how we implement \ourmethod system.~\Cref{fig:dust_block_diagram} shows the block diagram of \ourmethod. In this section, we detail how we search for the unionable tuples from the data lake and align their columns with the query table's columns.
% For these tasks, we primarily inherit existing techniques~\cite{2023_fan_starmie, 2022_khatiwada_alite} with necessary modifications.
In the next section, we cover our novel Unionable Tuple Diversification Algorithm~(\cref{section:unionable_tuple_diversification}).
%tuple representation model~(\cref{section:tuple_representation}) and our novel tuple diversification algorithm~(\cref{section:tuple_diversification}).

\rjm{This repeats what is already said in Section 3.  We aren't modifying table union search so I would remove this or remove from 3 -- the only important thing is that union search makes use of indices to achieve sublinear performance.}

\subsection{Table Search}
A simple baseline solution to search for unionable tuples may index some unionability information about each data lake tuple in the pre-processing phase and query over the created index in the query phase. However, the data lakes could contain an enormous number of tuples that are not practical to index.
Intuitively, the data lake tables that are unionable with the query table can contribute to the tuples that are unionable with the query table.
So, as shown in~\cref{fig:dust_block_diagram}, to search for unionable tuples, we search for the tables from the data lake that are unionable with the query table~(\cref{line:tsearch}). 
The table search technique could be either threshold-based (the query and the data lake tables are considered unionable if their unionability score exceeds a given threshold L) or top-L-based (returns data lake tables that have top-L unionability scores with the query table). Based on the technique, we provide L, which could be a threshold value or a positive integer, as a parameter. For instance, in our implementation, we use Starmie, a recent state-of-the-art table union search technique~\cite{2023_fan_starmie} which is top-L based.
The tuples from all the searched tables form the set of unionable tuples.


\rjm{again very repetitious with 3.  My suggestion is combine into 3 -- just add to three the one or two extra sentences you have in 4 and move Example to Section 3}
\aamod{merged with section 3 contents.}

%In our implementation, we use an existing table search technique~\cite{2023_fan_starmie} that 
% aamod: explain this in experimental setup
\subsection{Column Alignment}
The table union search techniques return a set of data lake tables unionable with the query table. However, to add the unionable tuples to the query table, we need to know which columns of data lake tables to align with each query column~\cite{2023_khatiwada_santos, 2023_fan_starmie}. Recall that data lake tables may have inconsistent or missing column headers and hence, we cannot rely on them to align the columns~\cite{2022_khatiwada_alite}.
So, we apply the column alignment phase to determine aligning columns by using the state-of-the-art table integration technique~\cite{2022_khatiwada_alite}.

Our objective is to get the disjoint set of columns such that columns in each set are aligned together. Furthermore, as we want to add data lake tuples to the query table, we ensure that the selected sets of columns have a query column on them on which other data lake columns are aligned.
So, we first embed all query and data lake columns using their values. Over such embeddings, we apply hierarchical clustering to generate a dendrogram that shows all possible clusters of columns. 
Recall that no two columns from the same table could be aligned together. Therefore, we enforce a constraint during clustering that prohibits clustering columns from the same table together.
Then an important decision is to select the number of clusters. For that, we compute a cluster quality score for each number of clusters and select the one that maximizes the quality.
We measure quality using Silhouette's coefficient~\cite{1987_rousseeuw_silhouttes} following the prior work~\cite{2022_khatiwada_alite}.

Note that we only need values from those data lake columns that align with at least one query table. Therefore, after getting all the clusters, we discard those that do not contain a column from the query table. This leaves us with a set of clusters, each with a query column and data lake columns that are aligned. Also, there could be query columns that do not align with any data lake column. For them, we get a singleton cluster having only a query column. 

%\aamod{todo: explain how ALITE's clustering method works and how we discard clusters after alite returns them to us.}

\begin{example}
\label{example:column_alignment}
    Consider Tables in~\cref{fig:park_tables} such that Table (a) is a query table and Tables (b), (c), and (d) reside in the data lake. Let us use the state-of-the-art table union search technique Starmie~\cite{2023_fan_starmie} to search for the top-2 unionable tables from the data lake. Then Tables (b) and (c) will be returned as two best unionable tables with Table (a). Next, we input columns of Tables (a), (b), and (c) into the column alignment phase where we get six clusters of columns. Specifically, the first cluster contains three \texttt{Park Name} columns from Tables (a), (b), and (c). The second cluster contains two \texttt{Supervisor} columns from Tables (a) and (b). The third cluster contains two \texttt{City} columns from Tables (a) and (b), and \texttt{Park City} column from Table (c). The fourth cluster contains two \texttt{Country} columns from Tables (a) and (b). We also get two singleton clusters with \texttt{Park Location} and \texttt{Park Phone} columns from Table (c). Since the last two clusters contain no columns from the query table, they are discarded. Then we are left with the first four clusters of columns that are assigned dummy column headers colA, colB, colC, and colD respectively.  
\end{example}
